From Coarse to Fine-grained Concept based Discrimination for Phrase Detection

Phrase detection requires methods to identify if a phrase is relevant to an image and localize it, if applicable. A key challenge for training more discriminative detection models is sampling negatives. Sampling techniques from prior work focus primarily on hard, often noisy, negatives disregarding the broader distribution of negative samples. Our proposed CFCD-Net addresses this through two novels methods. First, we generate groups of semantically similar words we call concepts (\eg, \{dog, cat, horse\} and \ \{car, truck, SUV\}), and then train our CFCD-Net to discriminate between a region of interest and its unrelated concepts. Second, for phrases containing fine-grained mutually-exclusive words (\eg, colors), we force the model to select only one applicable phrase for each region using our novel fine-grained module (FGM). We evaluate our approach on Flickr30K Entities and RefCOCO+, where we improve mAP over the state-of-the-art by 1.5-2 points. When considering only the phrases affected by our FGM module, we improve by 3-4 points on both datasets.

==> 7_ethics_rep.tex <==


\textbf{Code of Ethics Statement} Phrase detection methods like ours can help to better understand the content of images, which can be very useful for downstream tasks like image captioning and visual question answering. This can be extremely useful for some tasks like answering questions about images posed by people who have visual impairments, as many of these questions may not be answerable given the image content~\cite{Gurari_2018_CVPR}.  Methods performing well on phrase detection much better than methods developed for other phrase grounding tasks, as the primary difference is exactly to be able to identify if a phrase is present in an image in addition to localizing it.  However, these benefits also come with some risks, such as enabling some applications in tasks  like surveillance by allowing a user to quickly locate specific entities in a database of images.  We also note that although our approach provides significant performance improvements over the state-of-the-art, absolute performance on this task is still quite poor.  While this suggests there are ample opportunity for researchers to improve performance on this task, it also indicates that the results of these systems should not be trusted blindly.  We also note that Flickr30K Entities and COCO may contain personally identifiable information, but they remain standard benchmarks on phrase grounding tasks, making them an important comparison.


\textbf{Reproducibility Statement} We provide source code with the supplementary material to reproduce the results. Moreover, we provide extensive details for training the model and setting the hyper-parameters used in this study in Section \ref{sec:experiments}. Finally, all our reported results as indicated in Section \ref{sec:experiments} were averaged over 3 runs to ensure statistical significance. 

==> 8_supp_mod.tex <==


% \begin{table*}[t!]
%     \setlength{\tabcolsep}{2pt}
%     \centering
%     \caption{Phrase Localization accuracy comparison using Positive Phrase Augmentation (PPA) \cite{Plummer_2020} between prior work (SimNet w/CCA) and our model three novel components (EC, ER, and FGM). See Section~\ref{supp_phrase_loc} for discussion.}

%     \begin{tabular}{l|cc}
%         \midrule
%         & \multicolumn{1}{|c}{Flickr30K Entities}  &  \multicolumn{1}{|c}{RefCOCO+} \\
%         \midrule
%         SimNet w/CCA & 66.8 &  59.5\\
%         PFP-Net (CR)  & 58.8 & 57.6 \\
%         PFP-Net (CR+ER)  & 58.9 &  57.7\\
%         PFP-Net (CR+ER+FGM) & 60.3 & 58.3 \\
%         \midrule
%     \end{tabular}
%     %\vspace{-12mm}
%     \label{loc_ppa}
% \end{table*}


% However, to be complete, we report localization performance of our model without PPA in Table~\ref{loc_no_ppa} and with PPA in Table~\ref{loc_ppa}. We note that our methods' localization numbers are on par with previous work, with the only exception of when PPA is applied on Flickr30K. We would argue that this is likely due, in part, to the fact that the PPA augmentations are noisy, as \cite{Plummer_2020} themselves acknowledged. For example, using PPA augmentation on Flickr30K, any region labeled as “swimmers head cap” would also be labeled as a positive for “roof” or “jacket,” although these are clearly incorrect associations. Since our work more accurately distinguishes between phrases, we would more likely label the correct image region for such spurious associations. 



% \begin{table}[t!]
%     \caption{Detailed results for the phrase-based sentence-to-image retrieval benchmark. We rank image using Eq. \ref{eq:image-sentence} and then compute  $Recall@K=1, 5, 10$ to evaluate the methods. Refer to Section \ref{sec:image-sentence} for discussion.}

%     \setlength{\tabcolsep}{2pt}
%     \centering
%     \begin{tabular}{l|cccc}
%         \midrule
%         & R@1 & R@5 & R@10 & Mean\\
%         \midrule
%         Deep CCA [2] & 6.98 & 18.77 & 25.94 & 17.23\\
%         CCA [16] & 12.12 & 26.33 & 33.19 & 23.88\\
%         FAOG [42] & 3.14 & 9.03 & 14.96 & 9.04\\
%         QA R-CNN + NPA [15] & 4.33	& 11.47	& 17.74 & 11.18 \\
%         PFP-Net (ours) & \textbf{16.12}& \textbf{31.82}&	\textbf{39.78} & \textbf{29.24}\\
%         EmbNet [38] &3.91 &	10.99&	16.88 & 10.59\\
%         QA R-CNN [15] & 4.04	& 11.54 & 17.56 & 11.04\\
%         CITE [29] & 4.57 &	12.11&	18.00 & 11.56\\
%         SimNet [38] & 4.41	& 11.47	& 17.68 & 11.18\\
%         SimNet + CCA [32] & 13.53	&27.72	&35.46 & 25.57\\
%         \midrule
%     \end{tabular}
%     %\vspace{+2mm}
%     \label{tab:image-sentence-recall}
% \end{table}




%We then compute a threshold for Positive/Negative Matches using a grid search on the validation set. 

% \section{Concept generation ablations}
% \label{supp_concept_generate_abl}

% As discussed in Section 3, we use visually coherent groups (concepts) to provide negative samples that cover a broad spectrum of the training distribution. As noted in Section 3.1, DBSCAN + ViCo result in concepts with the least amount of visual coherence noise. Thus, we expect this combination to have the best performance. To verify this claim, we  provide an ablation study that document the impact of varying the embedding/clustering algorithm combination on the CR component of our PFP model. The component is responsible for using the concepts as negative samples. For each combination, we select the clustering algorithm hyper parameters that produce the least visual coherence noise. As we can see in Table~\ref{cr_ab}, DBSCAN+ViCo perform the best on both datasets. 

% While other combinations have equal performance on Flickr30k entities,  their performance align in RefCOCO+ dataset  with our visual coherence noise metric. 

% More concretely, K-means overall perform worse than DBSCAN and ViCO improves performance on either of the clustering algorithms when compared to GLoVE. 

\section{BISON benchmark}
\label{sec:image-sentence-supp}
In Section \ref{sec:related} of our paper we used the BISON benchmark \cite{Hu2019BinaryIS} to demonstrate how good performance on phrase detection leads to improved downstream task performance (unlike the localization-only task evaluated in most prior work).  In this benchmark, the model is asked to select the caption that best fits an image from a pair of semantically similar images.  Formally, given input image $I$ and and a set of noun phrases representing a the caption $S$, we would use a scoring function (\ie, a phrase grounding method) to measure the relationship between each phrase $S_{p_i}$, \ie, $\text{PhraseScore}(S_{p_i}, I)$.  Then, we compute the Image-Caption score $\text{ImgScore}(S, I)$ as follows: 

\begin{equation}
  \text{ImgScore}(S, I) = \frac{1}{|S|} \sum_{i=0}^{|S|} \text{PhraseScore}(S_{p_{i}}, I)
  \label{eq:image-sentence}
\end{equation}

\noindent We rank images for a given caption using Eq.~(\ref{eq:image-sentence}), then select the image with the bigger score.



 \begin{table*}[t!]%{\textwidth}
    \setlength{\tabcolsep}{3pt}
        \centering
        \begin{tabular}{rlcccccccc}
        \toprule
         &  & \multicolumn{4}{c}{Flickr30K Entities} & \multicolumn{4}{c}{RefCOCO+} \\ \midrule
         &  & zero- & few- & \multicolumn{1}{c}{com-} &  & zero- & few- & \multicolumn{1}{c}{com-} &  \\
         & \#Train Samples & shot & shot & \multicolumn{1}{c}{mon} & mean & shot & shot & \multicolumn{1}{c}{mon} & mean \\ \midrule
        \multicolumn{1}{l}{} & MDETR \cite{Kamath_2021_ICCV} & 1.6 & 2.6 & \multicolumn{1}{c}{8.0} & 4.0 & 1.4 & 2.8 & \multicolumn{1}{c}{11.0} & 5.0 \\
        \multicolumn{1}{l}{} & GLIP \cite{li2021grounded} & 4.3 & 6.8 & \multicolumn{1}{c}{13.7} & 8.3 & 1.9 & 4.4 & \multicolumn{1}{c}{12.6} & 6.3 \\
        \multicolumn{1}{l}{} & CCA \cite{Plummer_2020} & 8.9 & 10.7 & \multicolumn{1}{c}{18.9} & 12.9 & 5.7 & 8.3 & \multicolumn{1}{c}{20.9} & 11.7 \\
         & SimNet w/CCA \cite{Plummer_2020} & 9.4 & 11.2 & \multicolumn{1}{c}{19.8} & 13.5 & 6.2 & 10.3 & \multicolumn{1}{c}{20.5} & 12.3 \\ \midrule
         & +NCC & 10.6 & 12.1 & \multicolumn{1}{c}{20.4} & 14.3 & 6.2 & 10.3 & \multicolumn{1}{c}{21.8} & 12.8 \\
         & +NPA & 10.3 & 12.4 & \multicolumn{1}{c}{20.8} & 14.5 & 5.9 & 10.5 & \multicolumn{1}{c}{23.6} & 13.3 \\
         & +NPA+NCC & 10.7 & 12.7 & \multicolumn{1}{c}{21.4} & 15.0 & 6.4 & 10.5 & \multicolumn{1}{c}{23.8} & 13.5 \\
         & CFCD-Net (+ NPA + NCC + FGM) & \textbf{11.0} & \textbf{13.4} & \multicolumn{1}{c}{\textbf{21.7}} & \textbf{15.4} & \textbf{6.5} & \textbf{10.5} & \multicolumn{1}{c}{\textbf{24.2}} & \textbf{13.8} \\ \bottomrule
        \end{tabular}
     \caption{ mAP split by frequency of training instances where  \textbf{augmented positive phrases (PPA)} from \cite{Plummer_2020} is used for evaluation. The table compares our model three components (NPA, NCC, and FGM) to state of the art (SimNet w/CCA). See Section \ref{sec:results_discussion} for discussion}
    \label{tb:main_results_ppa}
\end{table*}


\begin{table}[t!]
    \setlength{\tabcolsep}{2pt}
    \centering
    \caption{Phrase Localization accuracy of prior work SimNet w/CCA and our model three components: NPA, NCC, FGM. Section~\ref{phrase-loc-supp} for discussion.}
    \begin{tabular}{lcc}
    \toprule
     & \begin{tabular}[c]{@{}c@{}}Flickr30K \\ Entities\end{tabular} & \begin{tabular}[c]{@{}c@{}}Ref\\ COCO+\end{tabular} \\ \midrule
    SimNet w/CCA & 71.9 & 57.5 \\
    +NPA & 70.6 & 56.3 \\
    +NPA+CR & 70.3 & 55.9 \\
    PFP-Net(+NPA+CR+FGM) & 70.3 & 55.9 \\ \bottomrule
    \end{tabular}   
    \label{loc_no_ppa}
     \vspace{-2mm}
\end{table}


\section{Positive Phrase Augmentation (PPA)}
\label{ppa-supp}

Table \ref{tb:main_results_ppa} reports the performance of CFCD-Net using positive phrase augmentation (PPA) \cite{Plummer_2020}, which reduces annotation sparsity by pairing ground truth phrases with plausible positive phrases using WordNet \cite{10.1145/219717.219748}. We note that PPA does not change the relative gains of the detection methods, but obtains higher absolute performance.


\section{Phrase localization performance}
\label{phrase-loc-supp}

As discussed in Section \ref{sec:related}, we note that localization and detection performance are not causally related. However, to be complete, we report localization performance of our model in Table~\ref{loc_no_ppa}. We note that our methods' localization numbers are on par with previous work. 



\begin{table}[t!]
    \caption{\textbf{Dataset annotations' false negative rate.} See Section~\ref{supp_datasets} for more details.}

    \setlength{\tabcolsep}{2pt}
    \centering
    \begin{tabular}{lc}
    \toprule
     & False \\ 
     & Negative\% \\ 
     \midrule
    Referit \cite{KazemzadehOrdonezMattenBergEMNLP14} & 74\% \\
    Visual Genome \cite{krishnavisualgenome} & 72\% \\
    Flickr30k Entities \cite{7410660} & 31\% \\
    RefCOCO+  \cite{10.1007/978-3-319-46475-6_5}& 40\% \\ \bottomrule
    \end{tabular} 

    \vspace{-1mm}
    \label{false_neg}
\end{table}


\section{Evaluation dataset selection}
\label{supp_datasets}

The sparsity of phrase detection datasets annotations poses significant challenges on evaluation. Real world datasets annotations can not cover all the possible positive cases. For example, a region annotated with only the phrase \textit{blue shirt} can also be correctly labeled with \textit{clothing}. \citet{Plummer_2020} attempted to mitigate this problem by introducing Positive Phrase Augmentations (PPA) where structures like WordNet \cite{10.1145/219717.219748} were used to derive additional positive samples. However, this problem is not limited to issues with synonyms. Phrases might have different structures but can convey the same meaning (\eg frisbee that is round vs a round frisbee), While the authors of Flickr30K \cite{7410660} limited the structure of their annotations to mitigate this problem, this is not the case for datasets like Visual Genome \cite{krishnavisualgenome} or Referit \cite{KazemzadehOrdonezMattenBergEMNLP14} therefore, their validity for phrase detection evaluation is not clear. To quantitatively document this issue, we sampled 30 random phrases from each dataset and considered the top 5 most similar phrases using the visual based language representation ViCo \cite{gupta2019vico}. For each of these top 5 phrases, we manually counted the number of false negatives. We report the average results in Table~\ref{false_neg}. Note that both Referit and Visual Genome suffer from significantly higher false negative rates than Flickr30k Entities. Thus, they are not viable evaluation datasets for phrase detection. We instead use Flickr30k Entities and  RefCOCO+ \cite{10.1007/978-3-319-46475-6_5} which was collected using the same underlying game as Referit but  with improved data collection standards. Thus the phrases were more appearance focused and concise as evident in the lower false negative rate Table~\ref{false_neg}.




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

